Stable Rank Normalization for Improved Generalization in Neural Networks and GANs

Exciting new work on the generalization bounds for neural networks (NN) given by Neyshabur et al. , Bartlett et al. closely depend on two parameter-depenedent quantities: the Lipschitz constant upper-bound and the stable rank (a softer version of the rank operator). This leads to an interesting question of whether controlling these quantities might improve the generalization behaviour of NNs. To this end, we propose stable rank normalization (SRN), a novel, optimal, and computationally efficient weight-normalization scheme which minimizes the stable rank of a linear operator. Surprisingly we find that SRN, inspite of being non-convex problem, can be shown to have a unique optimal solution. Moreover, we show that SRN allows control of the data-dependent empirical Lipschitz constant, which in contrast to the Lipschitz upper-bound, reflects the true behaviour of a model on a given dataset. We provide thorough analyses to show that SRN, when applied to the linear layers of a NN for classification, provides striking improvements-11.3% on the generalization gap compared to the standard NN along with significant reduction in memorization. When applied to the discriminator of GANs (called SRN-GAN) it improves Inception, FID, and Neural divergence scores on the CIFAR 10/100 and CelebA datasets, while learning mappings with low empirical Lipschitz constants.

==> algorithms.tex <==
As discussed in~\cref{sec:background}, learning $\theta$ such that $f$ is L-\Gls{lip} is highly desirable in variety of machine learning tasks.
Various regularizations such as spectral normalization, orthonormal projection, grandient penalty, and gradient clipping are tailored to achieve this task, directly or indirectly.
In what follows, we first discuss the importance of learning low rank intermediate affine mappings in a \gls{nn} in order to learn functions with low {\em empirical} \Gls{lip} constant. Then, we propose a new normalization that achieve this task very efficiently.


\subsection{Relating Rank with the Empirical Estimate of the \Gls{lip} Constant}
\label{sec:rank}
Learning parameters such that the \Gls{lip} constant meets the upperbound (refer~\eqref{eq:lipboundNN}), implying $\norm{f}_{Lip} = \prod_{i=1}^l \sigma(\wmat_i)$ (assuming matrix 2-norm), is highly unlikely in practice as this would require all the singular vectors corresponding to the maximum singular values of each intermediate layer to perfectly align with each other. However, in practice, different layers learn different parameters resulting in an empirical estimate of the \Gls{lip} constant which is much lower than the stated upper bound %
Thus, the design of a normalization scheme to minimize the \Gls{lip} constant should be motivated, not just by the upper bound, but also by its influence on the empirical estimate of the \Gls{lip} constant. Here we show how reducing rank can greatly minimize the \Gls{lip} constant. 

Let us assume the simplest possible case of a \gls{nn} with two linear layers having parameters $\wmat_1$ and $\wmat_2$ (ignoring the biases as the same argument will be valid with them being part of the network as well). We further assume that both the matrices are of rank $k$ with singular values as $\sigma_1 \geq \cdots \geq \sigma_k$, and $\lambda_1 \geq \cdots \geq \lambda_k$, respectively. Let $P_i = \bfu_i \bfu_i^\top$ denote the orthonormal projection matrix corresponding to the $\bfu_i$ singular vector of $\wmat_1$. Similarly, we define $Q_i$ for $\wmat_2$. Note, these assumptions are just for the sake of clarity, the arguments provided below can easily be extended for any number of arbitrary matrices. Then, for any two samples $\bfx_i$ and $\bfx_j$ from the dataset, the empirical \Gls{lip} constant can be written as (refer \cref{eq:lipGlobal}):
\begin{align}
\frac{\norm{f(\bfx_i) - f(\bfx_j)}}{\norm{\Delta  \bfx}} &= \frac{\norm{\wmat_2 \wmat_1 (\Delta  \bfx)}}{\norm{\Delta  \bfx}} \\ \nonumber 
&= \frac{\norm{M (\Delta  \bfx)}}{ \norm{\Delta  \bfx}}
\end{align}
where, $M = \big( \sum_i \sum_j \lambda_i \sigma_j Q_i P_j \big)$, and $\Delta \bfx = \bfx_i - \bfx_j$. This estimate of the \Gls{lip} will be $\sigma_1 \lambda_1$ (the upper bound) if and only if $P_1 = Q_1$, which is highly unlikely in practice.  Therefore, instead of just looking into the maximum singular values, minimizing all the singular values will lead to better \Gls{lip} constant in practice. For example, assigning $\sigma_j = 0$, which in effect will reduce the rank of $\wmat_1$ by one, will nullify its influence on all future projections associated with $P_j$. In another words, all the $k$ projections (or paths) that would propagate the input via $P_j$ in order to contribute to the final output will be blocked. This, in effect, will reduce $\norm{M (\Delta  \bfx)}$, hence the empirical \Gls{lip} constant. In a more general setting, let there are $l$ linear layers each with $k_i$ singular values (for $i$-th layer), then, each singular value of a $j$-th layer can influence $\prod_{i=1}^{j-1} k_i \prod_{i=j+1}^{l} k_i$ many directions through which an input could be propagated. Thus, with low rank mappings, chances are very high that the empirical estimate of the \Gls{lip} constant will be low, which we validate through extensive experiments on real datasets. %



\subsection{Stable Rank Normalization}
As discussed in~\cref{sec:rank}, reducing rank is desirable in order to learn mappings with low empirical \Gls{lip} constant. Here we propose a normalization scheme, that, instead of directly minimizing the rank, minimizes the {\em stable rank} (discussed below) of a matrix. Stable rank is a  proxy to rank and is actually a lower bound on the true rank of the matrix. It also has the advantage of being easily computable and differentiable as we will see below. 
\paragraph{Stable Rank}
The stable rank of a matrix $\wmat$ is a soft version of the rank operator, and, unlike rank, is insensitive to small changes in the matrix. It is defined as \( \srank{\wmat} = \frac{\norm{\wmat}_\forb^2}{\norm{\wmat}_2^2} = \frac{\sum_{i}^r \sigma_i^2(\wmat)}{\sigma_1^2(\wmat)} \) where $r$ is the rank of the matrix. As both Frobenius and spectral norm are differentiable~(under some mild assumptions) stable rank is also differentiable. Also, \( \srank{\wmat} = \frac{\sum_{i}^r= \sigma_i^2(\wmat)}{\sigma_1^2(\wmat)} \le \frac{\sum_{i}^r \sigma_1^2(\wmat)}{\sigma_1^2(\wmat)}  = r\). Thus it also lower bounds the true rank of the matrix.


\paragraph{Difficulties with Normalizing the Stable Rank} Note, stable rank of a matrix is invariant to scaling, implying, $\srank{\wmat} = \srank{\frac{\wmat}{\eta}}$, for any $\eta \in \real$. Therefore, any normalization scheme that modifies $\wmat = \sum_i \sigma_i \bfu_i \bfv_i^{\top}$ to $\widehat{\wmat} = \sum_i \frac{\sigma_i}{\eta}  \bfu_i \bfv_i^{\top}$ will not allow normalizing stable rank. Examples of such schemes would be spectral normalization~\citep{miyato2018spectral} where $\eta = \sigma_1$, and Forbenius normalization where $\eta = \norm{\wmat}_\forb$. Note, ideally, the spectral normalization should result in $\widehat{\wmat} = \sum_i \bar{\sigma_i}  \bfu_i \bfv_i^{\top}$, where $\bar{\sigma_i} = 1$ if $\sigma_i \geq 1$, otherwise $\bar{\sigma_i} = \sigma_i$. Since this scheme, even though optimal, would require computing all $\sigma_i \geq 1$, thus, is of less practical importance when it comes to applying it to \gls{nn}. The approximation to it, as used in~\citet{miyato2018spectral}, requires computing only the largest singular value and can be efficiently computed using power method. This  makes it widely applicable in a variety of tasks related to \gls{nn}. Our approach to stable rank normalization, presented below, is also designed while keeping the computational efficiency in mind so that it can be widely used.

\paragraph{An Approach towards Stable Rank Normalization} For a given matrix $\wmat \in \real^{m \times n}$, we formulate the stable rank normalization problem as:
\begin{align}
\label{eq:srankProblem}
&\min_{\widehat{\wmat}} \norm{\wmat - \widehat{\wmat}}_\forb \nonumber \\
&\textit{s.t.} \quad \srank{\widehat{\wmat}} \leq r,
\end{align}
where, $r \in (0, \rank{\wmat}]$ is a user defined parameter.
An approach to solving this problem would be to relax it by taking the Lagrangian and performing gradient descent as both the Forbenius norm and the stable rank are differentiable in most cases\footnote{They might be undifferentiable when the singular values are degenerate but that is highly improbably in a computational scenario} w.r.t. $\widehat{\wmat}$. This solution is computationally intensive, and will be impractical if applied at each iteration of the optimization of a \gls{nn}. In what follows, we propose a rather simple approach, shown in \cref{alg:stablerankNorm1}, to approximate $\wmat$ into $\widehat{\wmat}$ such that $\srank{\widehat{\wmat}} = r$. Note, similar to the approximate spectral normalization~\cite{}, this approach also requires the top singular value and corresponding vectors, which can be efficiently computed using power method. 


\begin{algorithm}[t]
\caption{Spectral Normalization}
\label{alg:spectralNormOptimal}
\begin{algorithmic}[1]
\Require $\wmat \in \real^{m \times n}$, $s$ 
\State $\wmat_1 \gets \mathbf{0}$, $p \gets \min(m,n)$
\For {$k \in \{1, \cdots, p\}$}
\State $\{\bfu_k, \bfv_k, \sigma_k\} \gets SVD(\wmat, k)$
\Comment{perform power method to get $k$-th singular value}
\If{$\sigma_k \geq s$}
\State $\wmat_1 \gets \wmat_1 + s \; \bfu_k \bfv_k^{\top}$
\State $\wmat \gets \wmat - \sigma_k \; \bfu_k \bfv_k^{\top}$
\Else
\State break
\Comment{exit for loop}
\EndIf
\EndFor
\\
\Return $\wmat \gets \wmat_1 + \wmat$
\end{algorithmic}
\end{algorithm}







\begin{algorithm}[t]
\caption{Stable Rank Normalization (Greedy)}
\label{alg:stablerankNorm}
\begin{algorithmic}[1]
\Require $\wmat \in \real^{m \times n}$, $r$, $k$
\Ensure $p = \min(m,n)$ 
\State $\wmat_1 \gets \mathbf{0}$, $\beta  \gets \norm{\wmat}_\forb^2$, $\eta \gets 0$
\For {$i \in \{1, \cdots, k - 1\}$}
\State $\{\bfu_i, \bfv_i, \sigma_i\} \gets SVD(\wmat, i)$
\Comment{perform power method to get $i$-th singular value}
\If{$r \geq \br{\sigma_i^2 + \eta}/\sigma_1^2$}
\label{eq:stableIf}
\State $\wmat_1 \gets \wmat_1 + \sigma_i \bfu_i \bfv_i^{\top}$
\label{eq:greedyStep}
\State $\eta \gets  \eta + \sigma_i^2, \beta \gets  \beta - \sigma_i^2$
\Else
\State break
\Comment{exit for loop}
\EndIf
\EndFor
\State $\eta \gets r\sigma_1^2 - \eta$ \\
\Return $\wmat \gets \wmat_1 + \sqrt{\frac{\eta}{\beta}} (\wmat - \wmat_1)$
\label{eq:returnStep}
\end{algorithmic}
\end{algorithm}



In algorithm~\ref{alg:spectralNormOptimal} we present the optimal algorithm for minimizing the spectral norm for the sake of completeness.  Next, we will motivate our algorithm for minimizing stable rank.

Let $p = \min(m,n)$, then, for any $k \in \{1, \cdots, p\}$, we define $\wmat_1^k = \sum_{i=1}^k \sigma_i\bfu_i \bfv_i^\top$ and $\wmat_2^k = \sum_{i=k+1}^p \sigma_i\bfu_i \bfv_i^\top$. Let $\widehat{\wmat}$ be the matrix obtained using \cref{alg:stablerankNorm} with the stopping parameter $k$.

\begin{claim}
$\srank{\widehat{\wmat}} = r$.
\end{claim}
\begin{claim}
  The  matrix $\widehat{\wmat}$ will be of the form $\wmat_1^k + \gamma \wmat_2^k$ for all $k$ where $\gamma = \frac{\sqrt{r \sigma_1^2 - \norm{\wmat_1^k}_\forb^2}}{\norm{\wmat_2^k}_\forb}$.
\end{claim}

We are interested to see how $\norm{\wmat - \widehat{\wmat}}_\forb$ behaves as $k$ increases.

\begin{lem}
\label{prop:srnProperty}
  For a given matrix $\wmat \in \real^{m \times n}$ and desired stable rank $r \leq \min (m, n)$, increase in $k$ in Algorithm~(\cref{alg:stablerankNorm}  takes the estimated matrix farther away from the given $\wmat$ in terms of Forbenius norm i.e. $\norm{\wmat - \widehat{\wmat}}_\forb$ is minimized for $k=1$.
\end{lem}


\begin{proof}

 We know that $\widehat{\wmat} = \wmat_1^k + \gamma\wmat_2^k$
  
  Plugging the value of $\gamma$ and using the fact that $\norm{\wmat_2^k} \neq 0$, we can write
  \begin{align*} \norm{\wmat - \widehat{\wmat}}_\forb &= \br{1 - \gamma}\norm{\wmat_2^k}_\forb\\
                                                  &= \norm{\wmat_2^k} - \sqrt{r\sigma_1^2 - \norm{\wmat_1^k}_\forb^2}\\
                                                  &= \norm{\wmat_2^k} - \sqrt{r\sigma_1^2 - \norm{\wmat}_\forb^2+ \norm{\wmat_2^k}_\forb^2}\\
  \end{align*}
  By assumption that \(\srank{\wmat}\ge r\), we can write\[\norm{\wmat - \widehat{\wmat}}_\forb = f(\norm{\wmat_2^k}_\forb)= \norm{\wmat_2^k} - \sqrt{a + \norm{\wmat_2^k}_\forb^2}\] where $a\le 0$ for all $k$. $f$ is hence a monotonically decreasing function with respect to  $\norm{\wmat_2^k}_\forb$ and hence with $k$. This proves that $k=1$ is the optimal solution. 



\end{proof}

While Lemma~\ref{prop:srnProperty} is not a proof of optimality, it shows that any algorithm, which  returns a solution of the form $\wmat_1 +\gamma\wmat_2$ where $\wmat_1$ and $\wmat_2$ are as defined above, the optimal solution is $\wmat_2 = \wmat  - \sigma_1\vec{u}_1\vec{v}_1^\top$.  This gives us Algorithm~\ref{alg:stablerankNorm1}. It is easy to see that after one step of Algorithm~\ref{alg:stablerankNorm}, the returned $\widehat{\wmat}=\sigma_1\vec{u}_1\vec{v}_1^\top + \sigma_1\sqrt{\frac{r - 1}{\sum_{j=2}^2\sigma_j^2}}\br{\wmat - \sigma_1\vec{u}\vec{v}_1^\top}$   is exactly the same as the output of  Algorithm~\ref{alg:stablerankNorm1}.
\begin{algorithm}[t]
\caption{Stable Rank Normalization}
\label{alg:stablerankNorm1}
\begin{algorithmic}[1]
\Require $\wmat \in \real^{m \times n}, r$ 
\Ensure $1 \leq r \leq \min(m,n)$
\State $\bfu_1, \bfv_1, \sigma_1$
\Comment{perform power method to get top singular value and corresponding vectors}
\State $\wmat_1 = \sigma_1 \bfu_1 \bfv_1^{\top}$, $\wmat_2 = \wmat - \wmat_1$
\Comment{projection of $\wmat$ orthogonal to  $\bfu_1 \bfv_1^{\top}$}
\State $\eta = \frac{\sqrt{r-1}\sigma_1}{\norm{\wmat_2}_\forb}$
\State $\wmat_{SRN} = \sigma_1 \bfu_1 \bfv_1^{\top} + \eta \wmat_2$
\State return: $\wmat_{SRN}$, $\eta$
\end{algorithmic}
\end{algorithm}


Finally our objective is to minimize the spectral norm and the stable rank jointly. Thus we are trying to solve the following optimization problem.

\begin{align}
\label{eq:st_sp_rankProblem}
&\min_{\widehat{\wmat}} \norm{\wmat - \widehat{\wmat}}_\forb \nonumber \\
  &\textit{s.t.}\quad\srank{\widehat{\wmat}} \leq r;\enskip\norm{\widehat{\wmat}}_2 = 1
\end{align}
where, $r \in (0, \rank{\wmat}]$ is a user defined parameter.

To do this we combine the spectral normalization approach from~\citet{miyato2018spectral} and the stable rank minimization algorithm in~\ref{alg:stablerankNorm1}. From here on, by referring to stable rank normalization we refer to the joint problem in~\ref{eq:st_sp_rankProblem}.
\subsection{Final Algorithm}
Here we provide our final algorithm for applying stable rank
normalizing to each linear layer of a \Gls{nn}. Note that this also
includes the linear transformations present in a convolutional layer. On a high level, the algorithm first normalizes the spectral norm and then normalizes the stable rank while keeping the stable rank constant. Interestingly, the stable rank normalization algorithm in~\ref{alg:stablerankNorm1} doesn't require use to modify the largest singular value and hence the algorithm is quite easy to implement.
\begin{algorithm}
  \caption{\label{algo:snorm_norm} SGD with spectral and stable rank normalization }
  \begin{itemize}
  \item Initialize $\bfu_l\in \real^{d_l}~{\rm for}~l=1,\dots,L$ with a random vector (sampled from isotropic distribution).
  \item For each update and each layer $l$:
  \begin{enumerate}
  \item Apply power iteration method to a unnormalized weight $\wmat^l$:
  \begin{align}
      \bfv_l &\leftarrow (\wmat^{l})^{\top} \bfu_l/ \norm{(\wmat^{l})^{\top} \bfu_l}_2\\
	  \bfu_l &\leftarrow (\wmat^{l})^{\top} \bfv_l/ \norm{(\wmat^{l})^{\top} \bfv_l}_2\\
  \end{align}
  \item Calculate $\wmat_{\rm SN}$ with the spectral norm:
  \begin{align}
      \wmat_{\rm SN} = \wmat^ls_l / \sigma(\wmat^l), \; \sigma(\wmat^l)= \bfu_l^{\top} \wmat^l \bfv_l
  \end{align}
  \item Calculate the projection of $\wmat_\ell$ orthogonal to the maximum singular vectors:
  \begin{align}\label{eq:norm_stable}
    \widehat{\wmat} &= \wmat_{\rm SN}^l - \bfu_l \bfv_l^{\top}\\
      \wmat_{\rm SRM}^l &=   \widehat{\wmat} \frac{\sqrt{r_\ell -
                               1}}{\norm{\widehat{\wmat}}_{\forb}} +  \bfu_l \bfv_l^{\top}
  \end{align}
  \item Update $\wmat^l$ with \gls{sgd} on the mini-batch dataset $\mathcal{D}_M$ with a learning rate $\alpha$:
  \begin{align}
      \wmat^\ell \leftarrow \wmat^\ell - \alpha \nabla_{\wmat^\ell} L(\wmat_{\rm
    SRN}^\ell, \mathcal{D}_M)
  \end{align}
  \end{enumerate}
  \end{itemize}
\end{algorithm}





==> arxiv_Makefile <==
TOPTARGETS := all clean

SUBDIRS := $(wildcard ./arxiv/figs/*/.)

$(TOPTARGETS): $(SUBDIRS)
$(SUBDIRS):
	$(MAKE) -C $@ $(MAKECMDGOALS)




PAPER=main
ARX = arxiv
SHELL=/bin/zsh
#SHELL=/bin/bash



FIGS_SVG2=$(wildcard $(ARX)/figs/*.svg)
FIGS_PS2=$(FIGS_SVG2:%.svg=%.ps)
FIGS_PDF2=$(FIGS_PS2:%.ps=%.pdf)

./arxiv/figs/%.ps: $(ARX)/figs/%.svg  ## Figures for the manuscript
	inkscape -D -z --file=$< --export-ps=$@; \

./arxiv/figs/%.pdf: $(ARX)/figs/%.ps  ## Figures for the manuscript
	inkscape -D -z --file=$< --export-pdf=$@ --export-latex

all:  $(SUBDIRS)   $(FIGS_PDF2) arxiv/main.bbl


arxiv/main.bbl:   $(FIGS_PDF2)  ## Build full thesis (LaTeX + figures)
	cp -r *.tex arxiv/ 
	cp -r *.sty arxiv/
	cp -r *.bst arxiv/
	pdflatex  arxiv/$(PAPER) 
	#pdflatex --aux-directory=./ --output-directory=./  $(ARX)/$(PAPER) 
	bibtex $(PAPER)
	mv $(PAPER).bbl arxiv/
	#pdflatex --aux-directory=$(ARX)/ --updoutput-directory=./  $(ARX)/$(PAPER)

ARXIV_SET:
	mkdir -p arxiv
	mkdir -p arxiv/figs
	cd figs; \
	find . -name '*.svg' | cpio -updm ../$(ARX)/figs/; \
	find . -name 'Makefile' | cpio -updm ../$(ARX)/figs/; \
	cd ..

clean:
	rm arxiv/figs/*.svg
#clean:  ## Clean LaTeX and output figure files
#    rm -f *.nav *.snm *.out *.aux *.log *.fls *.blg *.bbl
#    rm -f $(FIGURES_PDF)

#watch:  ## Recompile on any update of LaTeX or SVG sources
#    @while [ 1 ]; do; inotifywait $(ALL); sleep 0.01; make all; done


.PHONY: $(TOPTARGETS) $(SUBDIRS)


==> iclr2020/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> new_experiment.tex <==



==> new_proof.tex <==
\section{Proof for Optimal Stable Rank Normalization}
\label{sec:optimalSrank}


In this section, we look at the exact problem we try to solve approximately through Algorithm~\ref{algo:spectralStable}.


\begin{thm}[~\cref{thm:srankOptimal} (in the main paper) ]
\label{thm:srankOptimal_app}
Given a real matrix $\wmat = \sum_{i=1}^p \sigma_i \bfu_i \bfv_i^\top$ with rank $p$, a spectral norm constraint $\sigma >0 $, and a target stable rank $r$ where $1 \leq r < \srank{\wmat}$, the optimal solution to the problem
\begin{align*}
& \min_{\widehat{\wmat}} \norm{\wmat - \widehat{\wmat}}_{\forb}^2  \\
& \textit{s.t.} \quad \srank{\widehat{\wmat}} = r,  \\
&\sigma_i\br{\wmat} = \sigma. 
\end{align*}
is $\wmathw_k = \gamma_1\wmat_{1} + \gamma_{2} \wmat_{2}$, where $\lambda_i$'s are the singular values of $\wmathw$, $\wmat_1 = \sum_{i=1}^{\mathrm{max}\br{1,k}} \sigma_i \bfu_i \bfv_i^\top$ and $\wmat_{2} = \sum_{i=\mathrm{max}\br{2,k+1}}^p \sigma_i \bfu_i \bfv_i^\top$. For simplification, we define $\gamma = \frac{\sqrt{r \sigma_1^2 - \norm{\wmat_1}_\forb^2}}{\norm{\wmat_2}_\forb}$. Then,
\begin{itemize}
\item[a)]  If $k=0$, $\gamma_2 = \dfrac{\gamma + r - 1}{r}$ and $\gamma_1 =  \dfrac{\gamma_2}{\gamma}$. Note, in this case, $\norm{\wmat_1}_{\forb}^2 = \sigma_1^2$, making \( \gamma = \frac{\sqrt{r-1} \sigma_1}{\norm{\wmat_2}_\forb}\).
\item[b)] If $k\ge 1,~\gamma_1 = 1$ and $\gamma_2=\gamma$.
\item [c)] $\norm{\wmathw_k - \wmat}_\forb$ is monotonically increasing with $k$ for $k \geq 1$.
\end{itemize}
\begin{proof}
We provide a thorough proof with optimality and uniqueness guarantees in~\cref{sec:optimalSrank}. \puneet{We must talk about the positivity of $\gamma$. This is missing from the proof as well.}
\end{proof}
\end{thm}


